Effects of Human Avatar Representation in Virtual Reality on Inter-Brain Connection

Increasing advances in affordable consumer hardware and accessible software frameworks are now bringing Virtual Reality (VR) to the masses. Especially collaborative VR applications where different people can work together are gaining momentum. In this context, human avatars and their representations are a crucial aspect of collaborative VR applications as they represent a digital twin of the end-users and determine how one is perceived in a virtual environment. When it comes to the effect of avatar representation on the end-users of collaborative VR applications, so far mostly questionnaires have been used to assess the quality of avatar representations. A promising alternative to objectively measure the effect of avatar representation is the investigation of inter-brain connections during the usage of a collaborative VR application. However, the combination of immersive VR applications and inter-brain connections has not been fully researched yet. Thus, our work investigates how different human avatar representations (real (RL), full-body (FB), and head-hand (HH)) affect inter-brain connections. For this purpose, we have designed and conducted a hyperscanning study with eight pairs. The main results of our hyperscanning study show that the number of significant sensor pairs was the highest in the RL, medium in the FB, and lowest in the HH condition indicating that an avatar that looks more like a real human enables more significant sensor pairs to appear in an EEG analysis.

==> 4_Implementation.tex <==
\section{Implementation}
\label{sec:implementation}
In this Section, we present the implementation of \textit{VRACP} by motivating the choice of VR Device and Development Platform and presenting each component separately. The code of \textit{VRACP} is publicly available via GitHub\footnote{\url{https://github.com/iwowi-projects/VRACP}}.

\subsection{VR Device and Development Platform}
Based on our conceptual decisions, we decided to use the \textit{Oculus Quest 2} as our main VR device. It comes with one HMD and a pair of hand controllers, has integrated speakers and microphones, provides 6 degrees of freedom, and is not dependent on further external hardware like PCs.
Concerning the development platform, we opted to use \textit{Unity 3D} which is a very popular game engine for developing 2D, 3D, AR, and VR games. It comes with many freely available plugins to enhance productivity and simplify programming. 

\subsection{Components}
\textbf{Virtual Environment}
Following the decision and design elements from Sec. \ref{sec:conceptual_solution}, we designed a realistic-looking office room. We relied on free external models and objects from the Unity \textit{Asset Store} \footnote{\url{https://assetstore.unity.com/}}, mainly furniture, tables, chair, decoration, plants, etc. The resulting office room can be divided into two areas: the first area contains the mentioned furniture without further functionality while the second area contains all the necessary areas to enable Scrum meetings and deals with its artifacts. 

\textbf{Virtual Character}
For the visual representation of the users' \textsc{Virtual Characters}, we decided to integrate seven male and female pre-rigged avatars from \textit{mixamo} \footnote{\url{https://www.mixamo.com/}}, an online avatar library, as they were free, human-like, full-body, and came with walking animations. In order to synchronize the physical hardware (HMD and controllers) with their virtual correspondings, we made use of the \textit{XR Interaction Toolkit} provided by Unity, a free package coming with pre-configured, platform-independent game objects to reduce development time. Concerning the interaction with the objects inside the environment, the package's \textit{Ray Interactor} was used which shoots a ray (line) from the user's hand. Whenever the ray reaches a valid target, the user can interact with the object. By this, unnecessary movement inside the room is reduced and the user can more easily interact with UI elements. \\
For the movement of the user, we added the \textit{Continuous move provider} and \textit{Snap turn provider} to the character. The user uses the left joystick to move and the right one to turn. The Inverse Kinematics aspect of the body was mainly provided by the \textit{Animation Rigging} package and its predefined components, where we only had to map the corresponding objects. For completion, each character has a nickname field above his head to better distinguish the people in the room and also a menu in front of the avatar where the user can make configurations, read a help text or leave the current room. Fig. \ref{fig:jeff_avatar} shows one male avatar with a body, nickname, and menu. 

\setlength{\belowcaptionskip}{-5pt}
\setlength{\intextsep}{10pt}
\begin{figure}[h]
\centering
\begin{minipage}{0.45\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{fig/AvatarMenu.JPG}
  \captionof{figure}{Male user represented through an avatar}
  \label{fig:jeff_avatar}
\end{minipage}
\hfill%
\begin{minipage}{0.45\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{fig/CollabIssueCard2.JPG}
  \captionof{figure}{\textit{Backlog Area}}
  \label{fig:megan_avatar}
\end{minipage}
\end{figure}

\textbf{Network Synchronization}
We required a system to enable multiplayer browsable rooms, the synchronization of the user's movement, voice chat, and sporadic events. We decided to use Exit Games' \textit{Photon Unity Networking} (PUN) \footnote{\url{https://www.photonengine.com/pun}}, a free software package for creating multiplayer-based games in Unity as it provided all the necessary functionality to fit our needs. In order to implement these features, according to the official documentation, it was only necessary to place specific predefined objects into the environment or attach them to the players. \\

\textbf{Artifacts}
We opted to use three-dimensional interactable objects for representing issues and sprints which are shown in Fig. \ref{fig:5_issue_card} and \ref{fig:5_sprint_card}. We designed the objects from scratch and put a canvas with all the relevant information on it. In order to make them grabbable and synchronized, it was only necessary to attach the required components from the \textit{XR Interaction Toolkit Package} and \textit{PUN2}. \\

\setlength{\belowcaptionskip}{-10pt}
\setlength{\intextsep}{5pt}
\begin{figure}[h]
\centering
\begin{minipage}{0.5\textwidth}
  \adjustimage{width=0.95\textwidth, left}{fig/IssueCard.JPG}
    \caption{3D Issue Card}
    \label{fig:5_issue_card}
\end{minipage}%
\begin{minipage}{0.5\textwidth}
  \adjustimage{width=0.95\textwidth, right}{fig/SprintCardNew.JPG}
    \caption{3D Sprint Box}
    \label{fig:5_sprint_card}
\end{minipage}
\end{figure}

\textbf{Areas}
The environment required different areas dedicated to a specific purpose for providing Scrum meetings and managing issues and sprints. These areas were either designed as a scrollable bookshelf with slots for issues/sprints or as a table on which the user can place an issue/sprint. The first design was used for the \textit{Backlog Area}, \textit{Board Area}, \textit{Sprint Area} and \textit{Sprint Issues Area}, whereas the second one was required by the \textit{Edit Issue Area}, \textit{Create Issue Area} and \textit{Create Sprint Area}. Two areas are shown in Fig. \ref{fig:collab_create_sprint} and \ref{fig:collab_edit_issue}. \\

\begin{figure}[h]
\begin{minipage}{0.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{fig/CollabCreateSprint.JPG}
  \captionof{figure}{Collaborative Sprint Creating in \textit{Create Sprint Area}}
  \label{fig:collab_create_sprint}
\end{minipage}
\hfill%
\begin{minipage}{0.5\textwidth}
  \centering
  \includegraphics[width=01\linewidth]{fig/CollabEditIssue.JPG}
  \captionof{figure}{Collaborative Issue Editing in \textit{Edit Issue Area}}
  \label{fig:collab_edit_issue}
\end{minipage}
\end{figure}

==> boxplot.tex <==

\begin{tikzpicture}
\begin{axis}[
    boxplot/draw direction=y,
    height=8cm,
    ymin=0.5, ymax=5.5,
    boxplot={
        %
        % Idea: 
        %  place the 
        %  group 1 at 0.3333 and 0.6666
        %  group 2 at 1.3333 and 1.6666
        %  group 3 at 2.3333 and 2.6666
        %  ...
        % in a formular:
        draw position={1/3 + floor(\plotnumofactualtype/2) + 1/3*mod(\plotnumofactualtype,2)},
        %
        % that means the box extend must be at most 0.33333 :
        box extend=0.3,
    },
    % ... it also means that 1 unit in x controls the width:
    x=1.4cm,
    % ... and it means that we should describe intervals:
    xtick={0,1,2,...,7},
    x tick label as interval,
    xticklabels={%
        {SP1\\{\tiny VR/Web}},%
        {SP2\\{\tiny VR/Web}},%
        {SP3\\{\tiny VR/Web}},%
        {SP4\\{\tiny VR/Web}},%
        {SP5\\{\tiny VR/Web}},%
        {SP6\\{\tiny VR/Web}},%
        {SP7\\{\tiny VR/Web}},%
    },
    x tick label style={
        text width=1.5cm,
        align=center
    },
]

\addplot+[color=edge_color,fill=vr_color,boxplot prepared={
			lower whisker=1, lower quartile=2.5,
			median=4, upper quartile=4,
			upper whisker=4}]
coordinates {};
\addplot[fill=web_color, boxplot]
table[row sep=\\,y index=0] {
data\\
1\\
2\\
3.5\\
4\\
5\\
};

\addplot[fill=vr_color]
table[row sep=\\,y index=0] {
data\\
1\\
2\\
3.5\\
4\\
5\\
};
\addplot[fill=web_color]
table[row sep=\\,y index=0] {
data\\
1\\
1.5\\
2\\
4\\
4\\
};

\addplot[fill=vr_color]
table[row sep=\\,y index=0] {
data\\
4\\
4\\
4\\
4.5\\
5\\
};
\addplot[fill=web_color]
table[row sep=\\,y index=0] {
data\\
1\\
1.5\\
2\\
3.5\\
5\\
};

\addplot[fill=vr_color]
table[row sep=\\,y index=0] {
data\\
2\\
2.5\\
3\\
4\\
4\\
};
\addplot[fill=web_color]
table[row sep=\\,y index=0] {
data\\
2\\
2\\
2.5\\
3\\
4\\
};

\addplot[fill=vr_color]
table[row sep=\\,y index=0] {
data\\
1\\
1.5\\
2\\
2.5\\
4\\
};
\addplot[fill=web_color]
table[row sep=\\,y index=0] {
data\\
1\\
2\\
3.5\\
4\\
5\\
};

\addplot[fill=vr_color]
table[row sep=\\,y index=0] {
data\\
1\\
1.5\\
2.5\\
4.5\\
5\\
};
\addplot[fill=web_color]
table[row sep=\\,y index=0] {
data\\
2\\
3\\
4\\
4.5\\
5\\
};

\addplot[fill=vr_color]
table[row sep=\\,y index=0] {
data\\
1\\
2\\
3\\
3.5\\
5\\
};
\addplot[fill=web_color]
table[row sep=\\,y index=0] {
data\\
2\\
2\\
3\\
4\\
4\\
};

\end{axis}
\end{tikzpicture}









\begin{figure}[H]

\begin{subfigure}{.3\textwidth}
    \centering
    \begin{tikzpicture}
		\begin{axis}[width=\textwidth,
		boxplot/draw direction=y,
		axis x line*=bottom,
		axis y line*=left,
        height=5cm,
		ymin=1,
		ymax=5,
        boxplot/every median/.style={very thick, solid},
		xtick={1,2},
		xticklabels={VR, Web},
		ylabel={SP1},
        ymajorgrids=true, major grid style={line width=0.1pt}
		]
		\addplot+[color=edge_color,fill=vr_color,boxplot prepared={
			lower whisker=1, lower quartile=2.5,
			median=4, upper quartile=4,
			upper whisker=4}]
        coordinates {};
		\addplot+[color=edge_color,fill=web_color,boxplot prepared={
			lower whisker=1, lower quartile=2,
			median=3.5, upper quartile=4,
			upper whisker=5}]
        coordinates {};
	   \end{axis}
	\end{tikzpicture}
\end{subfigure}
\hfill%
\begin{subfigure}{.3\textwidth}
    \centering
    \begin{tikzpicture}
		\begin{axis}[width=\textwidth,
		boxplot/draw direction=y,
		axis x line*=bottom,
		axis y line*=left,
        boxplot/every median/.style={solid}, 
        ymajorgrids=true, major grid style={line width=0.1pt},
        height=5cm,
		ymin=1,
		ymax=5,
		xtick={1,2},
		xticklabels={VR, Web},
		ylabel={SP2}
		]
		\addplot+[color=edge_color,fill=vr_color,boxplot prepared={
			lower whisker=1, lower quartile=2,
			median=3.5, upper quartile=4,
			upper whisker=5}]
        coordinates {};
		\addplot+[color=edge_color,fill=web_color,boxplot prepared={
			lower whisker=1, lower quartile=1.5,
			median=2, upper quartile=4,
			upper whisker=4}]
        coordinates {};
	   \end{axis}
	\end{tikzpicture}
\end{subfigure}%
\hfill%
\begin{subfigure}{.3\textwidth}
    \centering
    \begin{tikzpicture}
		\begin{axis}[width=\textwidth,
		boxplot/draw direction=y,
		axis x line*=bottom, axis y line*=left,
        height=5cm,
        boxplot/every median/.style={solid}, 
        ymajorgrids=true, major grid style={line width=0.1pt},
		ymin=1, ymax=5,
		xtick={1,2}, xticklabels={VR, Web},
		ylabel={SP3}
		]
		\addplot+[color=edge_color,fill=vr_color,boxplot prepared={
			lower whisker=4, lower quartile=4,
			median=4, upper quartile=4.5,
			upper whisker=5}]
        coordinates {};
		\addplot+[color=edge_color,fill=web_color,boxplot prepared={
			lower whisker=1, lower quartile=1.5,
			median=2, upper quartile=3.5,
			upper whisker=5}]
        coordinates {};
	   \end{axis}
	\end{tikzpicture}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
    \centering
    \begin{tikzpicture}
		\begin{axis}[width=\textwidth,
		boxplot/draw direction=y,
		axis x line*=bottom,
		axis y line*=left,
        height=5cm,
		ymin=1,
		ymax=5,
        boxplot/every median/.style={very thick, solid},
		xtick={1,2},
		xticklabels={VR, Web},
		ylabel={SP4},
        ymajorgrids=true, major grid style={line width=0.1pt}
		]
		\addplot+[color=edge_color,fill=vr_color,boxplot prepared={
			lower whisker=2, lower quartile=2.5,
			median=3, upper quartile=4,
			upper whisker=4}]
        coordinates {};
		\addplot+[color=edge_color,fill=web_color,boxplot prepared={
			lower whisker=2, lower quartile=2,
			median=2.5, upper quartile=3,
			upper whisker=4}]
        coordinates {};
	   \end{axis}
	\end{tikzpicture}
\end{subfigure}
\hfill%
\begin{subfigure}{.3\textwidth}
    \centering
    \begin{tikzpicture}
		\begin{axis}[width=\textwidth,
		boxplot/draw direction=y,
		axis x line*=bottom,
		axis y line*=left,
        boxplot/every median/.style={solid}, 
        ymajorgrids=true, major grid style={line width=0.1pt},
        height=5cm,
		ymin=1,
		ymax=5,
		xtick={1,2},
		xticklabels={VR, Web},
		ylabel={SP5}
		]
		\addplot+[color=edge_color,fill=vr_color,boxplot prepared={
			lower whisker=1, lower quartile=1.5,
			median=2, upper quartile=2.5,
			upper whisker=4}]
        coordinates {};
		\addplot+[color=edge_color,fill=web_color,boxplot prepared={
			lower whisker=1, lower quartile=2,
			median=3.5, upper quartile=4,
			upper whisker=5}]
        coordinates {};
	   \end{axis}
	\end{tikzpicture}
\end{subfigure}%
\hfill%
\begin{subfigure}{.3\textwidth}
    \centering
    \begin{tikzpicture}
		\begin{axis}[width=\textwidth,
		boxplot/draw direction=y,
		axis x line*=bottom, axis y line*=left,
        height=5cm,
        boxplot/every median/.style={solid}, 
        ymajorgrids=true, major grid style={line width=0.1pt},
		ymin=1, ymax=5,
		xtick={1,2}, xticklabels={VR, Web},
		ylabel={SP6}
		]
		\addplot+[color=edge_color,fill=vr_color,boxplot prepared={
			lower whisker=4, lower quartile=4,
			median=4, upper quartile=4.5,
			upper whisker=5}]
        coordinates {};
		\addplot+[color=edge_color,fill=web_color,boxplot prepared={
			lower whisker=1, lower quartile=1.5,
			median=2, upper quartile=3.5,
			upper whisker=5}]
        coordinates {};
	   \end{axis}
	\end{tikzpicture}
\end{subfigure}

\label{fig:6_social_presence_room_sharing}
\end{figure}
